The Leaky Pipeline in Physics Publishing

Women make up a shrinking portion of physics faculty in senior positions, a phenomenon known as a "leaky pipeline." While fixing this problem has been a priority in academic institutions, efforts have been stymied by the diverse sources of leaks. In this paper we identify a bias potentially contributing to the leaky pipeline. We analyze bibliographic data provided by the American Physical Society (APS), a leading publisher of physics research. By inferring the gender of authors from names, we are able to measure the fraction of women authors over past decades. We show that the more selective, higher impact APS journals have lower fractions of women authors compared to other APS journals. Correcting this bias may help more women publish in prestigious APS journals, and in turn help improve their academic promotion cases.

==> coverletter.tex <==
 
October 14, 2020

Dear Editors,

We are pleased to submit our manuscript titled “The Leaky Pipeline in Physics Publishing” for consideration of publication in the journal Physical Review Letters.
Our paper is an attempt to examine systemic gender biases in the physics community using bibliographic data provided by the American Physics Society (APS), the leading publishing of physics research. By genderizing the names of authors who published papers in APS journals over the many decades, we are able to quantify the representation of women in physics. We identify a gender gap, where the more prestigious journals publish fewer papers by women physicists. Our paper suggests the need to examine the editorial policies of the APS, especially of the high-impact journals.

Relevance to physics. Although our paper does not address a physics problem, it examines the practice of physics, and thus would be of interest to physicists.  Several papers published by Physical Review Letters were based on the same data we explore.

This work is not under consideration by any other journal. Below we list names, affiliations, and email addresses of a potential editor and five potential referees, all of whom are highly recognized and well qualified to judge this work.

We thank you for your consideration of our paper.
Sincerely,
The authors
 


